DyCL: Dynamic Neural Network Compilation Via Program Rewriting and Graph Optimization

DL compiler's primary function is to translate DNN programs written in high-level DL frameworks such as PyTorch and TensorFlow into portable executables. These executables can then be flexibly executed by the deployed host programs. However, existing DL compilers rely on a tracing mechanism, which involves feeding a runtime input to a neural network program and tracing the program execution paths to generate the computational graph necessary for compilation. Unfortunately, this mechanism falls short when dealing with modern dynamic neural networks (DyNNs) that possess varying computational graphs depending on the inputs. Consequently, conventional DL compilers struggle to accurately compile DyNNs into executable code. To address this limitation, we propose \tool, a general approach that enables any existing DL compiler to successfully compile DyNNs. \tool tackles the dynamic nature of DyNNs by introducing a compilation mechanism that redistributes the control and data flow of the original DNN programs during the compilation process. Specifically, \tool develops program analysis and program transformation techniques to convert a dynamic neural network into multiple sub-neural networks. Each sub-neural network is devoid of conditional statements and is compiled independently. Furthermore, \tool synthesizes a host module that models the control flow of the DyNNs and facilitates the invocation of the sub-neural networks. Our evaluation demonstrates the effectiveness of \tool, achieving a 100\% success rate in compiling all dynamic neural networks. Moreover, the compiled executables generated by \tool exhibit significantly improved performance, running between $1.12\times$ and $20.21\times$ faster than the original DyNNs executed on general-purpose DL frameworks.

==> Preliminary/study.tex <==
\subsection{Study Question}


==> Table/overheads.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{0.5\textwidth}{!}{
     \begin{tabular}{cccccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{ID.}}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{Overheads}}} & \multicolumn{3}{c}{\textbf{Comlitation Overheads}} & \multicolumn{3}{c}{\textbf{Extra Percentage (\%)}} \\
          &       & \multicolumn{1}{l}{\textbf{TorchMobile}} & \multicolumn{1}{l}{\textbf{TVM (CPU)}} & \multicolumn{1}{l}{\textbf{TVM (GPU)}} & \multicolumn{1}{l}{\textbf{TorchMobile}} & \multicolumn{1}{l}{\textbf{TVM (CPU)}} & \multicolumn{1}{l}{\textbf{TVM (GPU)}} \\
    \midrule
    1     & 0.06  & 27.93  & 11.63  & 41.30  & 0.20  & 0.47  & 0.13  \\
    2     & 0.06  & 32.09  & 11.62  & 45.15  & 0.20  & 0.54  & 0.14  \\
    3     & 0.13  & 159.31  & 30.08  & 99.66  & 0.08  & 0.43  & 0.13  \\
    4     & 0.06  & 45.53  & 17.07  & 40.92  & 0.12  & 0.33  & 0.14  \\
    5     &       &       &       &       &       &       &  \\
    6     &       &       &       &       &       &       &  \\
    7     &       &       &       &       &       &       &  \\
    8     &       &       &       &       &       &       &  \\
    9     &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
}
  \label{tab:addlabel}%
\end{table}%


==> Text/application.tex <==
\section{Application}



==> Text/threat.tex <==
\section{Threat to Validity}

Our selection of the AdNN systems, namely, ShallowDeep, SkipNet, AttentionNet, and En-Decoder, might be a threat to
the \textit{external validity} of our experimental conclusions. 
We have tried to alleviate this threat by the following efforts:
(1) The AdNNs are very popular, which can be seen through the number of citations of the works (Table \ref{});
(2) The underlying DNN models are state-of-the-art models, which are used significantly;
(3) These systems differ from each other in terms of model architecture and functionality.
Therefore, our experimental conclusions should generally hold.


%although specific
%data could be inevitably different for other subjects.
%Our \textit{internal threat} mainly comes from our definition of different perturbation types. Our introduced perturbation may not always be grammatically correct (\eg inserting one character may result in an unknown token).
%However, as discussed in \secref{sec:background}, such perturbations may not be typical but exist in the real-world (\eg user typos, adversarial manner).Thus, it is meaningful to understand NMT systems efficiency degradation with such realistic perturbations.
